Adaptive Similarity Bootstrapping for Self-Distillation based Representation Learning

Most self-supervised methods for representation learning leverage a cross-view consistency objective i.e., they maximize the representation similarity of a given image's augmented views. Recent work NNCLR goes beyond the cross-view paradigm and uses positive pairs from different images obtained via nearest neighbor bootstrapping in a contrastive setting. We empirically show that as opposed to the contrastive learning setting which relies on negative samples, incorporating nearest neighbor bootstrapping in a self-distillation scheme can lead to a performance drop or even collapse. We scrutinize the reason for this unexpected behavior and provide a solution. We propose to adaptively bootstrap neighbors based on the estimated quality of the latent space. We report consistent improvements compared to the naive bootstrapping approach and the original baselines. Our approach leads to performance improvements for various self-distillation method/backbone combinations and standard downstream tasks. Our code is publicly available at https://github.com/tileb1/AdaSim.

==> chapters/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
        \item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}
\end{enumerate}

==> chapters/definitions.tex <==
% Define annotation commands
\newcommand{\Tim}[1]{\textcolor{magenta}{#1}}
\newcommand{\Thomas}[1]{\textcolor{blue}{#1}}
\newcommand{\Behzad}[1]{\textcolor{red}{#1}}
\newcommand{\Tinne}[1]{\textcolor{green}{#1}}



% Define math annotations
% \newcommand{\glob}{\bar{\boldsymbol{z}}}
% \newcommand{\dense}{\mathbf{Z}}
\newcommand{\objects}{\mathbf{O}}
\newcommand{\cost}{\mathbf{M}}
% \newcommand{\loc}{\boldsymbol{z}_{t,k}}
% \newcommand{\p}{\boldsymbol{p}}
\newcommand{\PP}{\mathbf{P}}
\newcommand{\Q}{\mathbf{Q}}
\newcommand{\Y}{\mathbf{Y}}
\newcommand{\M}{\mathbf{M}}
\newcommand{\mask}{\mathbf{H}}
\newcommand{\tmarg}{\mathbf{r}}
\newcommand{\omarg}{\mathbf{c}}
\newcommand{\cls}{\texttt{[CLS]}}
\newcommand{\model}{g}
\newcommand{\backbone}{f}
\newcommand{\head}{h}

% Define name annotations 
\newcommand{\mname}{\texttt{TBD}}
\newcommand{\vit}{\text{ViT}}
\newcommand{\dino}{\text{DINO}}
\newcommand{\mae}{\text{MAE}}
\newcommand{\ibot}{\text{iBOT}}
\newcommand{\beit}{\text{BEiT}}
\newcommand{\densecl}{\text{DenseCL}}
\newcommand{\resnet}{\text{ResNet}}
\newcommand{\soco}{\text{SoCo}}
\newcommand{\pixpro}{\text{PixPro}}
\newcommand{\resim}{\text{ReSim}}
\newcommand{\orl}{\text{ORL}}

==> tables/ablation_old.tex <==
\begin{table}[b]
\caption{\textbf{Ablation study over AdaSim specific hyperparameters.} The ablation is run over 800 epochs.} %The temperature $\tau$ (a) and support size $K$ (c) are run with 800 epochsThe window size $w$ ablation (b) is only run on 100 epochs due to compute constraints. \TODO{800 epochs}
    \begin{subtable}{0.5\textwidth}
    \centering
    \begin{tabular}{c|ccc c c}
        Temperature $\tau$ &  0.0 & 0.05 & 0.1 & \cellcolor{cyan!20} 0.2 & 0.4\\ %0.00625 & 0.0125 & 0.025
        \midrule
        $k$-NN & 68.4 & 68.8 & 69.0 & \cellcolor{cyan!20} \textbf{70.1} & 69.8\\ %& 68.7 & 68.7 & 69.0
        linear & 71.9 & 72.4 & 72.6 & \cellcolor{cyan!20} \textbf{73.3} & 73.2\\
    \end{tabular}
    \caption{Temperature $\tau$}
    \end{subtable}%
    
    \begin{subtable}{0.5\textwidth}
    \centering
    \begin{tabular}{c|cccc}
        % Window size $w$ &  1 & 10 & 25 & \textbf{50} \\
        % \midrule
        % ImageNet $k$-NN top-1 & 55.1 & 57.6 & 58.3 & 59.4\\
        % ImageNet $k$-NN top-5 & 77.2 & 79.2 & 80.0 & 80.5  \\
        Window size $w$ &  1 & \cellcolor{cyan!20} 10 & 50 \\
        \midrule
        $k$-NN & 69.3 & \cellcolor{cyan!20} \textbf{70.1} & 69.4\\
        linear & 72.6 & \cellcolor{cyan!20} \textbf{73.3} & 72.7\\
        %[69.09, 87.166]
    \end{tabular}
    \caption{Window size $w$}
    \end{subtable}%
    
    \begin{subtable}{0.5\textwidth}
    \centering
    \begin{tabular}{c|ccccc}
        Support size $K$ &  2 & \cellcolor{cyan!20} 3 & 5 & 10 & 20 \\
        \midrule
        $k$-NN & 69.4 & \cellcolor{cyan!20} \textbf{70.1} & 70.1 & 69.1 & 68.4\\
        linear & 72.8 & \cellcolor{cyan!20} \textbf{73.3} & 73.0 & 72.5 & 72.2 \\
    \end{tabular}
    \caption{Support size $K$}
    \end{subtable}%
    \label{tab:ablation_old}
\end{table}

==> tables/vitb16_in.tex <==
\begin{table}[h]
\centering
\caption{
\textbf{A larger backbone is pre-trained with AdaSim} and evaluated on the standard $k$-NN, and linear evaluation benchmarks. ``\collapse'' denotes collapse.
} \footnotesize
\resizebox{1\columnwidth}{!}{
\begin{tabular}{l c c c c c c}
\toprule
% && \multicolumn{8}{c}{Evaluation epoch} \\
% \cmidrule{3-10} 
% && \multicolumn{2}{c}{200} && \multicolumn{2}{c}{500} && \multicolumn{2}{c}{800} \\
% \cmidrule{3-4} \cmidrule{6-7} \cmidrule{9-10}
Method        & Model & Dataset & Epochs && $k$-NN & linear \\
% \midrule
\midrule
DINO-2   & ViT-B/16 & ImageNet-1k    & 800 && 69.2 & 73.5  \\
DINO-2 + NN & ViT-B/16 & ImageNet-1k & 800 && \collapse & \collapse \\
\rowcolor{cyan!20} DINO-2 + AdaSim & ViT-B/16 & ImageNet-1k & 800&&  \textbf{72.7} \textcolor{darkgreen}{(+ 3.5)} & \textbf{75.0} \textcolor{darkgreen}{(+ 1.5)} \\
\bottomrule
\end{tabular}
\label{table:vitb16_in}
}
\end{table}%

